Imaging Systematics and Clustering of DESI Main Targets

We evaluate the impact of imaging systematics on the clustering of luminous red galaxies (LRG), emission-line galaxies (ELG) and quasars (QSO) targeted for the upcoming Dark Energy Spectroscopic Instrument (DESI) survey. Using Data Release 7 of the DECam Legacy Survey, we study the effects of astrophysical foregrounds, stellar contamination, differences between north galactic cap and south galactic cap measurements, and variations in imaging depth, stellar density, galactic extinction, seeing, airmass, sky brightness, and exposure time before presenting survey masks and weights to mitigate these effects. With our sanitized samples in hand, we conduct a preliminary analysis of the clustering amplitude and evolution of the DESI main targets. From measurements of the angular correlation functions, we determine power law fits $r_0 = 7.78 \pm 0.26$ $h^{-1}$Mpc, $\gamma = 1.98 \pm 0.02$ for LRGs and $r_0 = 5.45 \pm 0.1$ $h^{-1}$Mpc, $\gamma = 1.54 \pm 0.01$ for ELGs. Additionally, from the angular power spectra, we measure the linear biases and model the scale dependent biases in the weakly nonlinear regime. Both sets of clustering measurements show good agreement with survey requirements for LRGs and ELGs, attesting that these samples will enable DESI to achieve precise cosmological constraints. We also present clustering as a function of magnitude, use cross-correlations with external spectroscopy to infer $dN/dz$ and measure clustering as a function of luminosity, and probe higher order clustering statistics through counts-in-cells moments.

==> data_availability_statement.tex <==
The data underlying this article were accessed from The Legacy Survey (\texttt{http://legacysurvey.org/}). The derived data generated in this research will be shared upon reasonable request to the corresponding author.

==> tables/cic_elg.tex <==
\begin{tabular}{cccccccc}
%\hline
\multicolumn{8}{c}{\textbf{ELG}} \\
\hline
Cell width & $\bar{N}$ & $\sigma^2$ & $\frac{\langle (N - \bar{N})^3 \rangle}{\sigma^3}$ & $\frac{\langle (N - \bar{N})^4 \rangle}{\sigma^4}$ & $\overline{w}_2$ & $\overline{w}_3$ & $\overline{w}_4$ \\
%\hline
$0.010^{\circ}$ & $0.2350 \pm 0.0030$ & $0.290 \pm 0.010$ & $5.0 \pm 1.2$ & $90 \pm 47$ & $1.10 \pm 0.27$ & $30 \pm 15$ & $2000 \pm 1100$ \\
$0.014^{\circ}$ & $0.4530 \pm 0.0058$ & $0.630 \pm 0.034$ & $5.0 \pm 1.5$ & $110 \pm 56$ & $0.90 \pm 0.21$ & $19.0 \pm 9.4$ & $800 \pm 520$ \\
$0.019^{\circ}$ & $0.870 \pm 0.011$ & $1.40 \pm 0.10$ & $6.0 \pm 1.8$ & $120 \pm 61$ & $0.70 \pm 0.16$ & $12.0 \pm 5.7$ & $400 \pm 230$ \\
$0.027^{\circ}$ & $1.690 \pm 0.022$ & $3.20 \pm 0.30$ & $7.0 \pm 2.0$ & $140 \pm 67$ & $0.50 \pm 0.12$ & $7.0 \pm 3.4$ & $200 \pm 100$ \\
$0.037^{\circ}$ & $3.260 \pm 0.042$ & $7.30 \pm 0.79$ & $7.0 \pm 2.2$ & $160 \pm 75$ & $0.380 \pm 0.088$ & $4.0 \pm 1.9$ & $80 \pm 49$ \\
$0.052^{\circ}$ & $6.290 \pm 0.080$ & $17.0 \pm 1.9$ & $7.0 \pm 2.2$ & $150 \pm 72$ & $0.260 \pm 0.055$ & $1.90 \pm 0.92$ & $30 \pm 18$ \\
$0.072^{\circ}$ & $12.10 \pm 0.15$ & $37.0 \pm 3.7$ & $6.0 \pm 1.8$ & $110 \pm 54$ & $0.170 \pm 0.030$ & $0.80 \pm 0.35$ & $7.0 \pm 4.6$ \\
$0.100^{\circ}$ & $23.40 \pm 0.30$ & $83.0 \pm 5.6$ & $5.0 \pm 1.2$ & $70 \pm 30$ & $0.110 \pm 0.013$ & $0.30 \pm 0.11$ & $1.60 \pm 0.92$ \\
$0.139^{\circ}$ & $45.30 \pm 0.57$ & $192.0 \pm 3.3$ & $4.00 \pm 0.50$ & $50 \pm 11$ & $0.0720 \pm 0.0036$ & $0.110 \pm 0.021$ & $0.40 \pm 0.12$ \\
$0.193^{\circ}$ & $87.0 \pm 1.1$ & $460 \pm 24$ & $3.40 \pm 0.25$ & $34.0 \pm 3.4$ & $0.0490 \pm 0.0018$ & $0.0480 \pm 0.0058$ & $0.110 \pm 0.019$ \\
$0.268^{\circ}$ & $169.0 \pm 2.1$ & $1200 \pm 170$ & $3.0 \pm 1.0$ & $30 \pm 15$ & $0.0350 \pm 0.0049$ & $0.030 \pm 0.013$ & $0.050 \pm 0.038$ \\
$0.373^{\circ}$ & $326.0 \pm 3.9$ & $3100 \pm 760$ & $3.0 \pm 1.7$ & $30 \pm 24$ & $0.0260 \pm 0.0065$ & $0.020 \pm 0.014$ & $0.030 \pm 0.034$ \\
$0.518^{\circ}$ & $628.0 \pm 7.3$ & $9000 \pm 3000$ & $3.0 \pm 2.1$ & $30 \pm 28$ & $0.0200 \pm 0.0071$ & $0.010 \pm 0.013$ & $0.020 \pm 0.027$ \\
$0.720^{\circ}$ & $1210 \pm 14$ & $30000 \pm 11000$ & $3.0 \pm 2.3$ & $30 \pm 29$ & $0.0170 \pm 0.0071$ & $0.010 \pm 0.010$ & $0.020 \pm 0.020$ \\
$1.000^{\circ}$ & $2340 \pm 25$ & $80000 \pm 39000$ & $2.0 \pm 2.2$ & $20 \pm 25$ & $0.0140 \pm 0.0068$ & $0.0070 \pm 0.0079$ & $0.010 \pm 0.012$ \\
\hline
\end{tabular}

==> tables/cic_lrg.tex <==
%\begin{tabular}{cccccccc}
\begin{tabular}{cccccccc}
\hline
\multicolumn{8}{c}{\textbf{LRG}} \\
\hline
Cell width & $\bar{N}$ & $\sigma^2$ & $\frac{\langle (N - \bar{N})^3 \rangle}{\sigma^3}$ & $\frac{\langle (N - \bar{N})^4 \rangle}{\sigma^4}$ & $\overline{w}_2$ & $\overline{w}_3$ & $\overline{w}_4$ \\
%\hline
$0.010^{\circ}$ & $0.0490 \pm 0.0019$ & $0.0550 \pm 0.0023$ & $7.50 \pm 0.23$ & $260 \pm 35$ & $2.410 \pm 0.014$ & $250 \pm 18$ & $88000 \pm 8100$ \\
$0.014^{\circ}$ & $0.0950 \pm 0.0036$ & $0.1120 \pm 0.0047$ & $7.30 \pm 0.35$ & $340 \pm 49$ & $1.870 \pm 0.022$ & $146.0 \pm 9.4$ & $40000 \pm 3400$ \\
$0.019^{\circ}$ & $0.1840 \pm 0.0069$ & $0.2320 \pm 0.0097$ & $7.50 \pm 0.45$ & $410 \pm 58$ & $1.420 \pm 0.025$ & $81.0 \pm 4.3$ & $16000 \pm 1200$ \\
$0.027^{\circ}$ & $0.350 \pm 0.013$ & $0.490 \pm 0.020$ & $8.10 \pm 0.48$ & $470 \pm 55$ & $1.060 \pm 0.025$ & $45.0 \pm 1.5$ & $6200 \pm 300$ \\
$0.037^{\circ}$ & $0.680 \pm 0.026$ & $1.050 \pm 0.042$ & $9.10 \pm 0.45$ & $550 \pm 44$ & $0.780 \pm 0.024$ & $24.90 \pm 0.21$ & $2520 \pm 21$ \\
$0.052^{\circ}$ & $1.320 \pm 0.050$ & $2.290 \pm 0.086$ & $10.00 \pm 0.38$ & $620 \pm 29$ & $0.560 \pm 0.020$ & $13.10 \pm 0.15$ & $990 \pm 26$ \\
$0.072^{\circ}$ & $2.550 \pm 0.096$ & $5.10 \pm 0.18$ & $10.10 \pm 0.22$ & $617.0 \pm 4.3$ & $0.390 \pm 0.015$ & $6.30 \pm 0.21$ & $360 \pm 28$ \\
$0.100^{\circ}$ & $4.90 \pm 0.19$ & $11.40 \pm 0.36$ & $9.200 \pm 0.090$ & $500 \pm 22$ & $0.270 \pm 0.012$ & $2.80 \pm 0.13$ & $110 \pm 12$ \\
$0.139^{\circ}$ & $9.50 \pm 0.36$ & $26.00 \pm 0.75$ & $7.550 \pm 0.016$ & $330 \pm 20$ & $0.1820 \pm 0.0086$ & $1.090 \pm 0.066$ & $27.0 \pm 3.5$ \\
$0.193^{\circ}$ & $18.40 \pm 0.70$ & $61.0 \pm 1.6$ & $5.710 \pm 0.016$ & $190 \pm 12$ & $0.1260 \pm 0.0063$ & $0.410 \pm 0.028$ & $5.80 \pm 0.83$ \\
$0.268^{\circ}$ & $35.0 \pm 1.3$ & $145.0 \pm 3.2$ & $4.070 \pm 0.049$ & $95.0 \pm 6.9$ & $0.0880 \pm 0.0047$ & $0.150 \pm 0.012$ & $1.20 \pm 0.19$ \\
$0.373^{\circ}$ & $69.0 \pm 2.6$ & $359.0 \pm 6.0$ & $2.790 \pm 0.093$ & $45.0 \pm 4.2$ & $0.0620 \pm 0.0036$ & $0.0560 \pm 0.0060$ & $0.250 \pm 0.044$ \\
$0.518^{\circ}$ & $132.0 \pm 5.1$ & $906.0 \pm 8.7$ & $1.90 \pm 0.13$ & $21.0 \pm 2.6$ & $0.0440 \pm 0.0029$ & $0.0210 \pm 0.0031$ & $0.050 \pm 0.011$ \\
$0.720^{\circ}$ & $256.0 \pm 9.8$ & $2338.0 \pm 5.3$ & $1.30 \pm 0.14$ & $11.0 \pm 1.6$ & $0.0320 \pm 0.0024$ & $0.0080 \pm 0.0016$ & $0.0100 \pm 0.0028$ \\
$1.000^{\circ}$ & $490 \pm 19$ & $6110 \pm 99$ & $0.90 \pm 0.13$ & $6.0 \pm 1.1$ & $0.0230 \pm 0.0020$ & $0.00360 \pm 0.00083$ & $0.00230 \pm 0.00080$ \\
\hline
\end{tabular}

==> tables/cic_qso.tex <==
\begin{tabular}{cccccccc}
%\hline
\multicolumn{8}{c}{\textbf{QSO}} \\
\hline
Cell width & $\bar{N}$ & $\sigma^2$ & $\frac{\langle (N - \bar{N})^3 \rangle}{\sigma^3}$ & $\frac{\langle (N - \bar{N})^4 \rangle}{\sigma^4}$ & $\overline{w}_2$ & $\overline{w}_3$ & $\overline{w}_4$ \\
%\hline
$0.010^{\circ}$ & $0.02990 \pm 0.00011$ & $0.03700 \pm 0.00054$ & $18.0 \pm 1.6$ & $1500 \pm 290$ & $7.90 \pm 0.42$ & $2900 \pm 440$ & $1900000 \pm 420000$ \\
$0.014^{\circ}$ & $0.05780 \pm 0.00022$ & $0.0800 \pm 0.0018$ & $25.0 \pm 3.2$ & $3000 \pm 650$ & $6.70 \pm 0.43$ & $2300 \pm 410$ & $1500000 \pm 360000$ \\
$0.019^{\circ}$ & $0.11160 \pm 0.00042$ & $0.1820 \pm 0.0064$ & $36.0 \pm 5.7$ & $5000 \pm 1300$ & $5.70 \pm 0.44$ & $1800 \pm 370$ & $1100000 \pm 300000$ \\
$0.027^{\circ}$ & $0.21550 \pm 0.00081$ & $0.440 \pm 0.022$ & $49.0 \pm 8.9$ & $9000 \pm 2300$ & $4.70 \pm 0.44$ & $1300 \pm 310$ & $800000 \pm 230000$ \\
$0.037^{\circ}$ & $0.4160 \pm 0.0016$ & $1.080 \pm 0.077$ & $60 \pm 12$ & $12000 \pm 3400$ & $3.80 \pm 0.41$ & $900 \pm 240$ & $500000 \pm 150000$ \\
$0.052^{\circ}$ & $0.8030 \pm 0.0030$ & $2.70 \pm 0.25$ & $70 \pm 15$ & $13000 \pm 4200$ & $2.90 \pm 0.37$ & $600 \pm 170$ & $240000 \pm 85000$ \\
$0.072^{\circ}$ & $1.5510 \pm 0.0058$ & $6.70 \pm 0.76$ & $70 \pm 17$ & $12000 \pm 4200$ & $2.10 \pm 0.30$ & $300 \pm 100$ & $100000 \pm 38000$ \\
$0.100^{\circ}$ & $2.990 \pm 0.011$ & $16.0 \pm 2.1$ & $70 \pm 16$ & $10000 \pm 3300$ & $1.50 \pm 0.22$ & $170 \pm 54$ & $40000 \pm 13000$ \\
$0.139^{\circ}$ & $5.780 \pm 0.021$ & $39.0 \pm 5.2$ & $60 \pm 13$ & $7000 \pm 2300$ & $1.00 \pm 0.15$ & $80 \pm 24$ & $11000 \pm 4000$ \\
$0.193^{\circ}$ & $11.160 \pm 0.040$ & $90 \pm 12$ & $50 \pm 10$ & $5000 \pm 1500$ & $0.640 \pm 0.094$ & $34.0 \pm 9.9$ & $3000 \pm 1100$ \\
$0.268^{\circ}$ & $21.550 \pm 0.077$ & $210 \pm 27$ & $42.0 \pm 7.5$ & $3400 \pm 930$ & $0.400 \pm 0.055$ & $13.0 \pm 3.6$ & $700 \pm 250$ \\
$0.373^{\circ}$ & $41.60 \pm 0.15$ & $450 \pm 59$ & $32.0 \pm 5.4$ & $2000 \pm 510$ & $0.240 \pm 0.033$ & $4.0 \pm 1.2$ & $140 \pm 49$ \\
$0.518^{\circ}$ & $80.30 \pm 0.29$ & $1000 \pm 130$ & $23.0 \pm 3.7$ & $1000 \pm 260$ & $0.140 \pm 0.019$ & $1.40 \pm 0.38$ & $25.0 \pm 8.5$ \\
$0.720^{\circ}$ & $155.20 \pm 0.56$ & $2100 \pm 270$ & $16.0 \pm 2.5$ & $500 \pm 130$ & $0.080 \pm 0.011$ & $0.40 \pm 0.11$ & $4.0 \pm 1.4$ \\
$1.000^{\circ}$ & $300.0 \pm 1.1$ & $4500 \pm 570$ & $10.0 \pm 1.5$ & $230 \pm 54$ & $0.0460 \pm 0.0061$ & $0.120 \pm 0.031$ & $0.60 \pm 0.20$ \\
\hline
\end{tabular}
